Identification For Control Based on Neural Networks: Approximately Linearizable Models

This work presents a control-oriented identification scheme for efficient control design and stability analysis of nonlinear systems. Neural networks are used to identify a discrete-time nonlinear state-space model to approximate time-domain input-output behavior of a nonlinear system. The network is constructed such that the identified model is approximately linearizable by feedback, ensuring that the control law trivially follows from the learning stage. After the identification and quasi-linearization procedures, linear control theory comes at hand to design robust controllers and study stability of the closed-loop system. The effectiveness and interest of the methodology are illustrated throughout the paper on popular benchmarks for system identification.

==> templates/identif_short.tex <==
\section{Identification procedure}
\label{sec:identif}

This section details the implementation of the training procedure of the AL-SSNN model \eqref{eq:ssnn_flin}.



==> templates/illustrations_short.tex <==
\section{Illustrations of training results}

The effectiveness of the proposed identification procedure is demonstrated using two benchmarks: a Wiener-Hammerstein process and a three species prey-predator system.

\subsubsection{Wiener-Hammerstein}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{templates/simu_wh.png}
    \caption{Training results for the Wiener-Hammerstein system. Blue: real output measurements, Red: error between real output and LTI model, Yellow: error between real output and AL-SSNN model \eqref{eq:ssnn_flin}.}
    \label{fig:res_wh}
\end{figure}

A Wiener-Hammerstein system with unknown differential equations and state vector in $\mathbb{R}^6$ was identified using 188,000 data points. Figure \ref{fig:res_wh} illustrates the error between the simulated output of the AL-SSNN model \eqref{eq:ssnn_flin} and the real output data. Table \ref{tab:res_WH} compares the root-mean-squared errors (RMSE) of the proposed model against a LTI model and the generalized nonlinear model \eqref{eq:ssnn_schoukens}.

\begin{table}
    \centering
    \caption{Wiener-Hammerstein training results. Comparison of root-mean-squared error (RMSE) of the proposed model and two models from literature : generalized ssnn \eqref{eq:ssnn_schoukens} and LTI .}
    \begin{tabular}{c|ccc}
        RMSE & \begin{tabular}{c} AL-SSNN \\ (This work, Eq. \eqref{eq:ssnn_flin}) \end{tabular} &  \begin{tabular}{c} GR-SSNN \\ (Eq. \eqref{eq:ssnn_schoukens}) \end{tabular} & LTI\\ 
        \hline 
        Training & $5.3 \times 10^{-4}$ & $3.6 \times 10^{-4}$ &  $2.7 \times 10^{-2}$ \\
        Test & $5.5 \times 10^{-4}$ & $3.7 \times 10^{-4}$ & $2.8 \times 10^{-2}$
    \end{tabular}
    \label{tab:res_WH}
\end{table}

Results show that the AL-SSNN model performs better than the LTI model and achieves comparable accuracy to the state-of-the-art nonlinear identification. The performance depends on the weighting scalar $\gamma$ in \eqref{eq:cost_min_res}, balancing model precision and ease of control synthesis.

\subsubsection{Prey-Predator system}

We consider a discretized version of a three species prey-predator system of the form:
\begin{equation}
    \begin{aligned}
    &\frac{d{x}_1}{dt} = a_1 x_1 - b_1 x_1 x_2 - c_1 x_1 x_3 + d_1 u_1 ^2\\
    &\frac{d{x}_2}{dt} =  a_2 x_2 - b_2 x_1 x_2 - c_2 x_1 x_3 +d_2 u_2^2\\
    &\frac{d{x}_3}{dt} =  -e x_3 + f x_1 x_3 + g x_2 x_3 \\    
    \end{aligned}
\end{equation}

for which the output is the predator $x_3$. The two prey species $x_1$ and $x_2$ are actuated with $u_1^2$ and $u_2^2$. The parameters $a_i$, $b_i$, $c_i$, $d_i$, $e$, $f$ and $g$ represents the growth/death rates, the effect
of predation on the prey population, and the growth of
predators based on the size of the prey population.

A discretized three species prey-predator system was identified using 50,000 data points. Figure \ref{fig:res_pp3} and Table \ref{tab:res_pp3} show that the AL-SSNN model achieves similar accuracy to the generalized nonlinear model, while the LTI model fails to represent the dynamics accurately.

Table \ref{tab:sum_bo} presents the ratio between nonlinear and linear terms, demonstrating that the proposed approach reduces the norm of the nonlinear residual by at least one order of magnitude compared to the generalized nonlinear model \eqref{eq:ssnn_schoukens}.

For the Wiener-Hammerstein system, the average ratio $\frac{\|g_{n}(x,u)\|}{\|Ax+Bu\|}$ is $1.9 \times 10^{-4}$, while for the prey-predator system, it is $2.5 \times 10^{-2}$. These results confirm the effectiveness of the AL-SSNN model in minimizing the residual nonlinearity while maintaining accurate system representation.

\section{Illustrations of training results}

The effectiveness of the proposed identification procedure is illustrated thanks to two popular benchmarks for system identification, a Wiener-Hammerstein process and a three species prey-predator system. 

\subsubsection{Wiener-Hammerstein}





The Wiener-Hammerstein system is a block-oriented structure composed of a static nonlinearity between two LTI blocks. The underlying differential equations are considered as unknown, we only assume that the state vector is in $\mathbb{R}^6$, following system description \cite{schoukens2009wiener}. 

We seek to identify a AL-SSNN model \eqref{eq:ssnn_flin} from time domain input-output data measurements consisting in $188~000$ points available online\footnote{https://sites.google.com/view/nonlinear-benchmark/benchmarks/wiener-hammerstein}. The data set is decomposed into training (first $100~000$ points) and test (last $88~000$ points).

We compare the identification capabilities of the presented AL-SSNN model \eqref{eq:ssnn_flin} with the one of the generalized nonlinear model \eqref{eq:ssnn_schoukens} where the nonlinear function $f_{n}$ is unconstrained. Results are illustrated on figure \ref{fig:res_wh} that shows the error between the simulated output of the proposed model \eqref{eq:ssnn_flin} and the real output data. In addition, table \ref{tab:res_WH} gathers the root-mean-squared errors (RMSE) between real output measurements and our proposed model. We provide the RMS errors between the data and a LTI model and the generalized nonlinear model \eqref{eq:ssnn_schoukens} for comparison. 

The results indicate that the proposed identification method performs better than standard LTI model and reaches same order of magnitude compared to state-of-the-art nonlinear identification. Note that these results depend on the choice of the weighting scalar $\gamma$ in \eqref{eq:cost_min_res}, the coefficients used for testing are gathered in table \ref{tab:config_training}. Our approach performs equally well when $\gamma \rightarrow 0$, it is then a compromise to be found between the models precision and ease of use for control synthesis, keeping in mind that the inaccuracies of the model can be tackled by a closed loop control scheme. A detailed analysis of the influence of parameter $\gamma$ is given in next section in table \ref{tab:diff_gamma_pp}.








\iffalse

\subsubsection{Prey-Predator system}


for which the output is the predator $x_3$. The two prey species $x_1$ and $x_2$ are actuated with $u_1^2$ and $u_2^2$. The parameters $a_i$, $b_i$, $c_i$, $d_i$, $e$, $f$ and $g$ represents the growth/death rates, the effect
of predation on the prey population, and the growth of
predators based on the size of the prey population. Inspired by \cite{brunton2016sparse}, for the data generation, we force the system sinusoidally with $u_i(t) = A_i sin(t+\phi_i) + A_i sin(t/10+\phi_i)$ and generate $50~000$ data points from which we use the first half for training and second half for validation.

The identification results are illustrated on figure \ref{fig:res_pp3} and gathered in table \ref{tab:res_pp3}. It shows that the LTI is not able to represent faithully the underlying dynamics but the identification method proposed above (AL-SSNN, equation \eqref{eq:ssnn_flin}) achieves the same order of magnitude as the generalized nonlinear model used for comparison. In addition, the training procedure ensures that the residual nonlinearity norm $\|g_{n}(x,u)\|$ is minimized. If successful, one should get after training $\|g_{n}(x,u) \| \ll \|Ax+Bu \| $. This is confirmed by results in table \ref{tab:sum_bo} that presents the mean and maximum values of the ratio between the nonlinear and linear terms of equation \eqref{eq:ssnn_flin}. Results show an average ratio of $1.9 \times 10^{-4}$ for the Wiener-Hammerstein example and $2.5 \times 10^{-2}$ for the prey-predator system while it was only of $0.20$ and $0.75$ for the generalized nonlinear model \eqref{eq:ssnn_schoukens}. The proposed approach therefore divide by at least one order of magnitude the norm of the nonlinear residual.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{templates/simu_pp3.png}
    \caption{Training results for the prey-predator system.  Blue: output measurements, Red: error between real output and LTI model, Yellow: error between real output and AL-SSNN model  \eqref{eq:ssnn_flin}.}
    \label{fig:res_pp3}
\end{figure}

\begin{table}
    \centering
    \caption{Prey-predator training results. Comparison of root-mean-squared error (RMSE) of the proposed model and two models from literature : generalized ssnn \eqref{eq:ssnn_schoukens} and LTI.}
    \begin{tabular}{c|ccc}
        RMSE & \begin{tabular}{c} This work \\ (model \eqref{eq:ssnn_flin}) \end{tabular} &  \begin{tabular}{c} GR-SSNN \\ (model \eqref{eq:ssnn_schoukens}) \end{tabular} & LTI\\ \hline 
        Train & $9.5 \times 10^{-2}$ & $6.7 \times 10^{-2}$ & $1.9 $ \\
        Test & $9.3 \times 10^{-2}$ & $6.5 \times 10^{-2}$ &  $1.9 $
    \end{tabular}
    \label{tab:res_pp3}
\end{table}



\begin{table*}[t]
    \centering
    \caption{Summary of open-loop simulation results for both examples Wiener-Hammerstein (W.H., top) and prey-predator systems (P.P., bottom). Each row depicts the results for the work presented in the paper, AL-SSNN model \eqref{eq:ssnn_flin}, and the generalized version, GR-SSNN \eqref{eq:ssnn_schoukens}, for comparison.}
    \begin{tabular}{c|cc|cc|cc}
          & \multicolumn{2}{c|}{$\frac{\|f_{n}(x,u)\|}{\|Ax+Bu\|}$} 
 & \multicolumn{2}{c}{$\frac{\|g_{n}(x,u)\|}{\|Ax+Bu\|}$} & \multicolumn{2}{c}{$\frac{\|h_{n}(y)\|}{\|Ax+Bu\|}$} \\
         &  $\max $ & ${\tt mean} $ & $\max $ & ${\tt mean} $  & $\max $  & ${\tt mean} $ \\ \hline  
         \begin{tabular}{c}
             W.H., AL-SSNN  \\
             (this work, Eq. \eqref{eq:ssnn_flin}) 
        \end{tabular} & $-$ & $-$ &  $3.6 \times 10^{-3} $ & $1.9 \times 10^{-4}$ & $1.2$ & $5.6 \times 10^{-2}$  \\
        & & & & & &  \\
        W.H., GR-SSNN \eqref{eq:ssnn_schoukens} & $0.45 $ &  $0.20$ &  $-$ & $-$ &  $-$&  $-$  \\  \hline 
                \begin{tabular}{c}
             P.P., AL-SSNN  \\
             (this work, Eq. \eqref{eq:ssnn_flin}) 
        \end{tabular} & $-$ & $-$ & $0.85 $ & $2.5 \times 10^{-2}$ & $25.16$ & $1.00 $  \\
        & & & & & &  \\
        P.P., GR-SSNN \eqref{eq:ssnn_schoukens} & $5.01 $ &  $0.75$  & $-$ & $-$ &  $-$ &  $-$
    \end{tabular}
    \label{tab:sum_bo}
\end{table*}

\fi

==> templates/intro_short.tex <==
\section{Introduction}

\subsection{Context and Related Works}

Data-driven methods are increasingly important in automatic control \cite{alamir2022learning}. However, temporal correlation in dynamical systems data can reduce the efficiency of control-oriented learning algorithms \cite{sznaier2020control}. Control-oriented learning takes different forms but one can find among others: the identification of linear parameter varying (LPV) approximation of nonlinear models \cite{verhoek2022}, the use of Koopman theory to learn a linear representation of a nonlinear system \cite{lusch2018deep} or learning-based model predictive control \cite{hewing2020learning}. 

We consider a plant described by an unknown discrete-time nonlinear state-space model:

\begin{equation}
    \begin{aligned}
    x(t+1) &= f(x(t),u(t)) \\
    y(t) &= Cx(t) 
    \end{aligned}
    \label{eq:modelNL}
\end{equation}

A neural state-space model approximates $f$ using a neural network $f_n$. Including an explicit linear part improves nonlinear model identification, which has been proven in \cite{schoukens_initvieux} to improve training :

\begin{equation}
    \begin{aligned}
    x(t+1) &= Ax(t)+Bu(t)+f_{n}(x(t),u(t)) \\
    y(t) &= Cx(t) 
    \end{aligned}
    \label{eq:ssnn_schoukens}
\end{equation}

Recent research focuses on robustness and stability analysis of neural models, often using incremental quadratic constraints and LMI certificates \cite{fazlyab2020safety,hashemi2021certifying}. These can also be included in training by adding a barrier term in the loss function \cite{pauli2022neuralSDP} or using projection-based algorithms \cite{yin_stability_2021}. Challenges in optimization have led to strategies like backtracking line search \cite{revay2020convex} to ensure the logdet term is well-defined or direct parameterization of network weights \cite{revay2024ren}.

This paper presents a strategy imposing a specific structure on the neural network to facilitate feedback-linearizing control law design, simplifying stability analysis and control design for nonlinear systems.

\subsection{Problem Statement and Contributions}

One approach to designing controllers for model \eqref{eq:ssnn_schoukens} is to treat the nonlinear function $f_{n}(x(t),u(t))$ as a modest, bounded disturbance compared to the linear part. This allows the use of extensive linear systems literature to design robust controllers that can handle these uncertainties. However, this approach has limitations. There's no guarantee that $f_{n}(x(t),u(t))$ will be small after identification, and minimizing $f_{n}$ may conflict with minimizing output simulation error.


%An alternative is to identify a linear time invariant (LTI) model, but this often fails to adequately represent complex system dynamics. Ideally, if we could make the dynamic behavior of model \eqref{eq:ssnn_schoukens} linear through feedback, controller design would be straightforward. However, conditions for exact feedback linearization are often challenging to meet in practice \cite{byrnes1989new}, especially for neural network architectures \cite{yesildirek_feedback_1995}.


%To address these challenges, we propose approximate feedback linearization. This approach aims to minimize the residual nonlinearity $f_{n}$ and decompose it into an input nonlinearity and an unavoidable modeling error. This decomposition offers significant advantages. The control law can more easily handle the input nonlinearity, while the training procedure focuses on minimizing the residual nonlinearity.

This paper introduces a control-oriented identification procedure, namely \textit{approximately feedback-linearizable state-space neural networks}, to identify system \eqref{eq:modelNL} with a given parameterized evolution equation such that the nonlinearity is explained as much as possible by a nonlinearity on the input. This ensures that the model is approximately linearizable by feedback. This work is an extension of previous work \cite{hacheICSC22} where the nonlinear system was assumed to be exactly feedback linearizable.

%\subsection{Notations}
%Standard notations are used: $x^T$, $M^T$ for transposes; $M = M^T > 0$ for symmetric positive definite matrices; $|x| = \sqrt{x^Tx}$ for Euclidian norm. $\mathcal{K}$-functions are continuous, strictly increasing with $f(0)=0$; $\mathcal{K}\infty$-functions additionally satisfy $\lim{x \rightarrow \infty} f(x) = \infty$. For discrete-time systems, $x_+$ denotes $x(t+1)$.



==> templates/rf_ssnn_short.tex <==
\section{Training of approximately feedback-linearizable neural state-space models}
Without loss generality, function $f_{n}(x,u)$ can be written as:
\begin{equation}
f_{n}(x,u) = B h_{n}(y) +  g_{n}(x,u)
\end{equation}
where $h_{n}(y)$ is an input nonlinearity and $g_{n}(x,u)$ is a residual nonlinearity.

\subsection{Definitions}
\textbf{Proposition 1. (AL-SSNN)} \textit{Approximately feedback-Linearizable State-Space Neural Networks} are nonlinear models with linear output:
\begin{equation}
    \begin{aligned}
    x_+ &= Ax+B\Big(u+h_{n}(y)\Big)+ g_{n}(x,u) \\
    y_\theta &= Cx
    \end{aligned}
    \label{eq:ssnn_flin}
\end{equation}
with parameters $\theta= \{A,B,C, h_{n}, g_{n} \}$ and neural networks $h_{n}$ and $g_{n}$.
~ \hfill $\blacksquare$

The approximately-linearizing control input is:
\begin{equation}
    u = v-h_{n}(y)
    \label{eq:quasi_lin_control}
\end{equation}
yielding the closed-loop model:
\begin{equation}
     \begin{aligned}
    x_+ &=  Ax+Bv +\omega \\
    y_\theta &= Cx
    \end{aligned}
    \label{eq:ssnn_flin_bf}
\end{equation}
where $\omega =  g_{n}(x,v-h_n(y))$.

Model parameters $\theta$ are obtained by minimizing the loss function :
\begin{equation}
\begin{aligned}
    \hat{\theta} = & \arg \min J_N(\theta) \\
    J_N(\theta) = & \frac{1}{N} \sum_{k=1}^N \Big( \big((y(k)-y_\theta(k)\big)^2   + \gamma g_{n}\big(x(k),u(k)\big)^2 \Big )
   \end{aligned}
    \label{eq:cost_min_res}
\end{equation}
where $\gamma$ weights the minimization of the nonlinearity against model precision.

\begin{figure}
    \centering   
    \includegraphics[width=0.6\textwidth]{templates/Schema_Flin_gen.png}
    \caption{Control architecture for 
 approximate feedback-linearization.}
    \label{fig:schema_rf_gen}
\end{figure}

\subsection{Network structure}

Functions $h_{n}(y)$ and $g_{n}(x,u)$ are both represented by a one-hidden-layer feed-forward neural network with nonlinear activation function with respectively $n_h$ and $n_g$ hidden neurons, and a linear output layer:
\begin{equation}
    \begin{aligned}
    h_{n}(y) &= W_h \sigma_h(W_{y} y + b_{y}) + b_h \\
    g_{n}(x,u) &= W_g \sigma_g(W_{x} x + W_{u} u + b_{x}) + b_g 
    \end{aligned}
\end{equation} 
where $\sigma_h : \mathbb{R}^{n_h} \rightarrow \mathbb{R}^{n_h}$ and $\sigma_g : \mathbb{R}^{n_g} \rightarrow \mathbb{R}^{n_g}$ are element-wise nonlinear activation functions that can be set independently but in the following we use hyperbolic tangent as activation function.

\subsection{Software Implementation}

The cost function \eqref{eq:cost_min_res} is nonlinear and not convex but its gradient can be computed efficiently, which makes the choice of gradient descent algorithm appropriate. The model is trained using algorithm implemented within the Matlab Deep Learning toolbox \cite{demuth1992neural} and Levenberg-Marquardt algorithm \cite{more1978levenberg}. %The training configurations for each example is detailed in table \ref{tab:config_training}, the identification method presented here involves only few parameters to tune and does not require the use of deep networks with large number of hidden neurons.

%The control-oriented architecture eventually slows down the identification procedure, as illustrated in table \ref{tab:config_training}. Training and simulations tests were carried out on a laptop with an Intel(R) Core(TM) i7 CPU at $1.80$ GHz x 4 with $32$GB of system memory. 

\subsection{Initialization}

 Inspired from \cite{schoukens_improved_2021}, the training procedure is iterative and starts by linear initialization, i.e. the AL-SSNN model \eqref{eq:ssnn_flin} is initialized as:
\begin{equation}
    \begin{aligned}
    x_+ &= A_0x+B_0u \\
    y_\theta &= C_0x 
    \end{aligned}
    \label{eq:lin_init}
\end{equation}
where matrices $A_0$, $B_0$ and $C_0$ are obtained using a linear identification algorithms, namely the subspace method implemented within the Matlab function {\tt ssest} together with {\tt n4sid} algorithm \cite{van1994n4sid}. In other words, functions $h_{n}$ and $g_{n}$ are initialized as $h_{n}(y) = 0$ and $g_n(x,u) = 0$. 

\subsection{Implementation of loss Function}

The goal is to minimize the ratio $\frac{|g_{n}(x,u)|}{|Ax+Bu|}$, making the nonlinear term negligible compared to the linear part. Due to computational challenges, we instead minimize $|g_{n}(x,u)|$ in the objective function \eqref{eq:cost_min_res} while keeping the output matrix $C$ fixed during training. This prevents the optimization from simultaneously scaling down $||x||$ and scaling up $C$, ensuring effective minimization of the desired ratio.


